Algorithms for Online Influencer Marketing

Influence maximization is the problem of finding influential users, or nodes, in a graph so as to maximize the spread of information. It has many applications in advertising and marketing on social networks. In this paper, we study a highly generic version of influence maximization, one of optimizing influence campaigns by sequentially selecting "spread seeds" from a set of influencers, a small subset of the node population, under the hypothesis that, in a given campaign, previously activated nodes remain "persistently" active throughout and thus do not yield further rewards. This problem is in particular relevant for an important form of online marketing, known as influencer marketing, in which the marketers target a sub-population of influential people, instead of the entire base of potential buyers. Importantly, we make no assumptions on the underlying diffusion model and we work in a setting where neither a diffusion network nor historical activation data are available. We call this problem online influencer marketing with persistence (in short, OIMP). We first discuss motivating scenarios and present our general approach. We introduce an estimator on the influencers' remaining potential -- the expected number of nodes that can still be reached from a given influencer -- and justify its strength to rapidly estimate the desired value, relying on real data gathered from Twitter. We then describe a novel algorithm, GT-UCB, relying on upper confidence bounds on the remaining potential. We show that our approach leads to high-quality spreads on both simulated and real datasets, even though it makes almost no assumptions on the diffusion medium. Importantly, it is orders of magnitude faster than state-of-the-art influence maximization methods, making it possible to deal with large-scale online scenarios.

==> variant.tex <==
% variant.tex

%\paragraph*{Related works.} In marketing, the rise of social networks led to a
%new form of marketing specifically dedicated to the promotion of brands and
%products online. Influence maximization (IM) is the data mining formalization of
%this problem where one tries to find the influent users / nodes in a graph so as
%to maximize the expected spread of the marketing campaign. A rich literature
%followed the seminal paper of Kempe et al.~\cite{kempe03}, focusing on scaling
%up algorithms to large graphs and dealing with various propagation
%models~\cite{goyal11,tang14,borgs14,ohsaka14,nguyen16}. In real life though,
%marketing firms frequently focus on influential people --~the
%\emph{influencers}~-- who can even be contractually bound by a sponsorship in
%exchange of the publication of promoting posts on their account. This new form
%of marketing is now referred to as the \emph{influencer marketing} and was
%largely discussed in the marketing literature~\cite{gillin07,duncan08, brown13}.
%The influence marketing problem was first considered in the IM literature under
%the online setting in~\cite{lagree17}.} 
In our study of the OIMP problem so far, a key assumption has been that the influencers
have a \emph{constant} tendency to activate their followers. This hypothesis may not be verified in certain situations, in which the moment influencers promote products
that do not align with their image (\emph{misalignement}) or persist in
promoting the same services (\emph{weariness}), they can expect their influence
to diminish~\cite{sletten17,lee17}. To cope with such cases of weariness, we propose in this section an extension to \algoname\ that incorporates the concept of
\emph{influencer fatigue}. %generated by the successive expositions to identical
%products / advertisings, that is, the case of weariness.

In terms of bandits, the idea of our extension is similar  in  spirit to the one of Levine et
al.~\cite{levine17}, who study a setting --~called \emph{rotting
bandits}~-- where each arm's value decays as a function of the number of times
it has been selected. We also mention the work of Lou\"edec et
al.~\cite{louedec16} in which the authors propose to take into account the
gradual obsolescence of items to be recommended while allowing new items to be
added to the pool of candidates. Importantly, the item's value is modeled by a
decreasing function of the number of steps since it was added to the pool of
items, whereas in our work --~and in that of~\cite{levine17}--, the value is a
function of the number of times \emph{the item has been selected}.

\subsection{Model adaptation}

Our variant to the OIMP with influencer fatigue can be reframed  as follows:

\begin{problem}[OIMP via \emph{rotting} influencers\label{def:problem-fatigue}]
  Given a set of influencers $[K]$, a \emph{budget} of $N$
  trials, a number $1 \leq L \leq K$ of influencers to be activated at each
  trial, the objective of online influence maximization with persistence
  (OIMP) via \emph{rotting} influencers is to solve the following optimization
  problem:
  $$
    \argmax_{I_n \subseteq [K], |I_n|=L, \forall 1\leqslant n\leqslant N}
    \mathbb{E}\left|\bigcup_{1\leqslant n \leqslant N} S(I_n) \right|,
  $$
  knowing the probability that, at its $s$-th selection, an influencer $k$
  $\in [K]$ activates some basic node $u$ is:
  $$
    p_s(u) = \gamma(s) p(u),
  $$
  for $\gamma: \mathbb{N} \to (0, 1]$ a \emph{known} non-increasing
  function and $p(u) \in [0,1]$.
\end{problem}

Our initial OIMP formulation can be seen as a special instance of the one via rotting influencers, where the non-increasing
function $\gamma$ --~referred to as the weariness function in the following~--
is the identity. We will follow the same strategy to solve it,  by estimating the remaining
potential of a given influencer by an adaptation of the Good-Turing estimator. What makes the problem more complex in this
rotting setting is the fact that hapaxes must now incorporate the round of their
activation.

\subsection{The \algonamefat~algorithm}

As we did previously, to simplify the analysis, we assume that the influencers
have \emph{non intersecting support}.  Let $n$ be the number of times a given
influencer has been selected and $S_1, \ldots, S_n$ the corresponding initiated
spreads. We redefine the remaining potential in the setting with influencer
fatigue as $R_n := \sum_{u \in A} \mathds{1}\{u \text{ never
activated}\} \gamma(n) p(u)$ where $p(u)$ is the probability that the influencer
activates node $u$, independently of the number of spreads initiated by the
influencer. Again, the remaining potential is equal to the expected number of
additional conversions at time $n$ given the nodes previously activated.  The
Good-Turing estimator adapted to the rotting setting is defined as follows:
$$
  \hat{R}_n = \sum_{u \in A} \frac{U^\gamma_n(u)}{n},
$$
where $U^\gamma_n(u) := \sum_{i < n} \mathds{1}\{X_0 = \ldots = X_{i-1} =
X_{i+1} = \ldots = X_{n-1} = 0, X_i = 1\} \frac{\gamma(n)}{\gamma(i)}$. In
short, if $i$ is the round at which a hapax has been activated, we reweight
it by the factor $\gamma(n) / \gamma(i)$ since we are interested in its
contribution at the $n$-th round. We now justify formally this estimator by
computing its bias.

Following principles from the bandit literature, the \algonamefat\ algorithm
relies on \emph{optimism in the face of uncertainty}. At each step (trial) $t$,
the algorithm selects the highest upper-confidence bound on the remaining
potential -- denoted by $b_k(t)$ -- and activates (plays) the corresponding
influencer $k$.  This algorithm achieves robustness against the stochastic
nature of the cascades, by ensuring that influencers who ``underperformed'' with
respect to their potential in previous trials may still be selected later on.
Consequently, \algoname\ aims to maintain a degree of \emph{exploration} of
influencers,  in addition to the \emph{exploitation} of the best influencers as
per the feedback gathered so far.

\begin{algorithm}
  \caption{ -- \algonamefat\ ($L = 1$)}
  \begin{algorithmic}[1]\small
    \REQUIRE{Set of influencers $[K]$, time budget $N$, fatigue function $\gamma$}
      \STATE{\textbf{Initialization:} play each influencer
        $k\in[K]$ once, observe the spread $S_{k,1}$, set $n_k=1$}
    \STATE{For each $k\in [K]$: update the reward $W=W\cup S_{k,1}$}
    \FOR{$t = K + 1, \ldots, N$}\label{alg:fatfor}
      \STATE Compute $b_k(t)$ for every influencer $k$
      \STATE Choose $k(t) = \argmax_{k \in [K]} b_k(t)$ \label{alg:fatoptimism}
      \STATE Play influencer $k(t)$ and observe spread $S(t)$
      \STATE Update cumulative reward: $W= W \cup S(t)$
      \STATE Update statistics of influencer $k(t)$: $n_{k(t)}(t+1) = n_{k(t)}(t) + 1$ and
      $S_{k,n_k(t)} = S(t)$.
    \ENDFOR   \label{alg:fatendfor}
  \RETURN $W$
  \end{algorithmic}
  \label{alg:fatgooducb}
\end{algorithm}

\hl{TODO: clean all this part to avoid repetitions}
Algorithm~\ref{alg:fatgooducb} presents the main components of \algonamefat\ for
the case $L=1$, that is, when a single influencer is chosen at each step. 

The algorithm starts by activating each influencer $k\in[K]$ once, in order to
initialize its Good-Turing estimator. The main loop  of \algonamefat\ occurs at
lines \ref{alg:fatfor}-\ref{alg:fatendfor}. Let $S(t)$ be the observed spread
at the trial $t$, and let $S_{k,s}$ be the result of the $s$-th diffusion
initiated at influencer $k$.  At every step $t > K$, we recompute for each
influencer $k \in [K]$ its index $b_k(t)$, representing the upper confidence
bound on the expected reward in the next trial. The computation of this index
uses the previous samples $S_{k,1},\ldots,S_{k,n_k(t)}$ and the number of times
each influencer $k$ has been activated up to trial $t$, $n_k(t)$. Based on the
result of Theorem~\ref{th:confidence_bounds}, the upper confidence bound is set
as:
\begin{align}\label{eq:fatucb}
  b_k(t) = \hat{R}_k(t) + \left(1+\sqrt{2}\right)\sqrt{\frac{\hat{\lambda}_k(t)
  \log(4t)}{n_k(t)}} + \frac{\log(4t)}{3n_k(t)},
\end{align}
where $\hat{R}_k(t)$ is the Good-Turing estimator and
$$
  \hat{\lambda}_k(t) := \frac{\gamma(n_k(t) + 1)}{n_k(t)} \sum_{s=1}^{n_k(t)}
  \frac{|S_{k,s}|}{\gamma(s)}
$$
is an estimator for the expected spread from influencer $k$.

Then, in line~\ref{alg:fatoptimism}, \algonamefat\ selects the influencer $k(t)$
with the largest index, and initiates a cascade from this node. The feedback
$S(t)$ is observed and is used to update the cumulative reward set $W$. Note
that $S(t)$ provides only the Ids of the nodes that were activated, with no
information on \emph{how} this diffusion happened in the hidden diffusion
medium. Finally, statistics associated to the chosen influencer $k(t)$ are
updated.

